Probing-RAG: Self-Probing to Guide Language Models in Selective Document Retrieval

Retrieval-Augmented Generation (RAG) enhances language models by retrieving and incorporating relevant external knowledge. However, traditional retrieve-and-generate processes may not be optimized for real-world scenarios, where queries might require multiple retrieval steps or none at all. In this paper, we propose a Probing-RAG, which utilizes the hidden state representations from the intermediate layers of language models to adaptively determine the necessity of additional retrievals for a given query. By employing a pre-trained prober, Probing-RAG effectively captures the model's internal cognition, enabling reliable decision-making about retrieving external documents. Experimental results across five open-domain QA datasets demonstrate that Probing-RAG outperforms previous methods while reducing the number of redundant retrieval steps.

==> TABLES/datasets.tex <==
% \begin{table}[ht]
% \small
% \begin{tabular}{lll}
% \hline
%           & \multicolumn{1}{c}{No Retrieval}& \multicolumn{1}{c}{Single Retrieval} \midrule
% Correct   & \begin{tabular}[c]{@{}l@{}}Query: What race track in the midwest hosts a 500 mile race eavery May?\\ Rationale: The Indianapolis 500 is a 500-mile (800 km) automobile race...\\ Pred: Indianapolis Motor Speedway\\ \\ Label: Indianapolis Motor Speedway\\ Acc: 1\end{tabular} & 

% \begin{tabular}[c]{@{}l@{}}Query: Were Scott Derrickson and Ed Wood of the same nationality?\\ Passages: \{Related passage 1, ..., Related passage 5\}\\ Rationale: Scott Derrickson is an American film director, screenwriter...\\ Pred: Yes\\ \\ Label: Yes\\ Acc: 1\end{tabular} 
% \midrule
% \midrule
% Incorrect & \begin{tabular}[c]{@{}l@{}}Query: When was Poison's album "Shut Up, Make Love" released?\\ Rationale: The album "Shut Up, Make Love" was released in ...\\ Pred: 1990\\ \\ Label: 2000\\ Acc: 0\end{tabular}  

% & \begin{tabular}[c]{@{}l@{}}Query: Are Random House Tower and 888 7th Avenue both used for real estate?\\ Passages: \{Related passage 1, ..., Related passage 5\}\\ Rationale: Random House Tower is a 40-story skyscraper in...\\ Pred: Yes\\ \\ Label: No\\ Acc: 0\end{tabular}     \\ \hline
% \end{tabular}

% \label{tab:dataset}
% \end{table}


